Measuring Nearby Star Forming Regions with the VLBA: from the Distance to the Dynamics

This thesis is part of a large ongoing effort to determine the distance and structure of all star-forming regions within several hundred parsecs of the Sun using radio-interferometric observations. The main goals of this thesis were: (1) Find the mean distance to the two best-studied nearby regions of low-mass star-formation (Taurus and Ophiuchus) with accuracies (a few percent or better) one to two orders of magnitude better than the present values, (2) Explore the structure and dynamics of these star-forming regions, and (3) Study the stars themselves.

==> tab-performance.tex <==
\begin{deluxetable}{cccccc}
%\rotate
\tabletypesize{\scriptsize}
\tablecolumns{6}
\tablewidth{0pc}
\tablecaption{Typical Performance Parameters at 86.2 GHz\label{tab-performance}}
\tablehead{
\colhead{Antenna}                              &
\colhead{Nominal Frequency}                    &
\colhead{Typical}                              &
\colhead{Typical}                              &
\colhead{Typical}                              &
\colhead{Baseline Sensitivity\tablenotemark{a}}\\
\multicolumn{1}{c}{}                           &
\multicolumn{1}{c}{Range}                      &
\multicolumn{1}{c}{Zenith $SEFD$}              &
\multicolumn{1}{c}{Zenith Gain}                &
\multicolumn{1}{c}{Zenith $T_{\rm sys}$}        &
\multicolumn{1}{c}{$\Delta S^{\rm 512, 30 s}$}  \\
\multicolumn{1}{c}{}                           &
\multicolumn{1}{c}{[GHz]}                      &
\multicolumn{1}{c}{[Jy]}                       &
\multicolumn{1}{c}{[K Jy$^{-1}$]}              &
\multicolumn{1}{c}{[K]}                        &
\multicolumn{1}{c}{[mJy]}                      }
\startdata
BR & 80.0 - 90.0 & 3500 & 0.039 & 135 & 55      \\%
NL & 80.0 - 96.0 & 4900 & 0.055 & 270 & 65      \\%
FD & 80.0 - 96.0 & 3600 & 0.034 & 120 & 55      \\%
LA & 80.0 - 90.0 & 3100 & 0.051 & 160 & $\cdots$\\%
PT & 80.0 - 96.0 & 4100 & 0.024 & 100 & 55      \\%
KP & 80.0 - 96.0 & 4600 & 0.025 & 110 & 60      \\%
OV & 80.0 - 96.0 & 5800 & 0.020 & 100 & 65      \\%
MK & 80.0 - 96.0 & 4100 & 0.023 & 100 & 55      \\%
\enddata
\tablenotetext{a}{Baseline to LA is assumed.}
\end{deluxetable}



==> tab-young.tex <==
\begin{deluxetable}{llll}
%\rotate
\tabletypesize{\scriptsize}
\tablecolumns{4}
\tablewidth{0pc}
\tablecaption{Observations of protostars\label{tab-young}}
\tablehead{
\colhead{Stars    }&
\colhead{Band     }&
\colhead{Range    }&
\colhead{Emission }}
\startdata
Young & Near infrared    & $3.5 \mu m \lesssim \lambda \lesssim 0.8 \mu m$ & thermal continua, vibrational lines\\%
      & Optical          & $0.8 \mu m \lesssim \lambda \lesssim 0.4 \mu m$ & molecular/atomic lines\\%
      & Near ultraviolet & $0.4 \mu m \lesssim \lambda \lesssim 0.1 \mu m$ & molecular/atomic lines\\%
      & Far ultraviolet  & $0.1 \mu m \lesssim \lambda \lesssim 15 n m$    & atomic lines, continua\\%
      & X-ray            & $15 n m \lesssim \lambda \lesssim 0.1 n m$      & inner shell atomic lines\\%
\\[-0.2cm]
\hline
\\[-0.2cm]
Very young & Radio          & $50 m \lesssim \lambda \lesssim 5 mm$          & non-thermal continua, rotational lines\\
           & Millimiter     & $5 mm \lesssim \lambda \lesssim 1mm$           & rotational lines, dust\\
           & Sub-millimiter & $1 mm \lesssim \lambda \lesssim 0.35 mm$       & rotational lines, dust\\
           & Far infrared   & $350 \mu m \lesssim \lambda \lesssim 20 \mu m$ & rotational lines\\
           & Mid infrared   & $20 \mu m \lesssim \lambda \lesssim 3.5 \mu m$ & vibrational lines\\
\enddata
\end{deluxetable}

